Automating Robot Failure Recovery Using Vision-Language Models With Optimized Prompts

Current robot autonomy struggles to operate beyond the assumed Operational Design Domain (ODD), the specific set of conditions and environments in which the system is designed to function, while the real-world is rife with uncertainties that may lead to failures. Automating recovery remains a significant challenge. Traditional methods often rely on human intervention to manually address failures or require exhaustive enumeration of failure cases and the design of specific recovery policies for each scenario, both of which are labor-intensive. Foundational Vision-Language Models (VLMs), which demonstrate remarkable common-sense generalization and reasoning capabilities, have broader, potentially unbounded ODDs. However, limitations in spatial reasoning continue to be a common challenge for many VLMs when applied to robot control and motion-level error recovery. In this paper, we investigate how optimizing visual and text prompts can enhance the spatial reasoning of VLMs, enabling them to function effectively as black-box controllers for both motion-level position correction and task-level recovery from unknown failures. Specifically, the optimizations include identifying key visual elements in visual prompts, highlighting these elements in text prompts for querying, and decomposing the reasoning process for failure detection and control generation. In experiments, prompt optimizations significantly outperform pre-trained Vision-Language-Action Models in correcting motion-level position errors and improve accuracy by 65.78% compared to VLMs with unoptimized prompts. Additionally, for task-level failures, optimized prompts enhanced the success rate by 5.8%, 5.8%, and 7.5% in VLMs' abilities to detect failures, analyze issues, and generate recovery plans, respectively, across a wide range of unknown errors in Lego assembly.

==> sec/related_work.tex <==
\section{Related Work}
\subsection{Robot Failure Detection and Recovery}
Robot failure detection and recovery are critical tasks for increasing human trust in human-robot collaboration~\cite{khanna2023user}, enabling non-expert users to assist robots during failure scenarios~\cite{das2021semantic, shi2024yell, zha2023distilling}, and allowing robots to self-correct their failures~\cite{xiong2024aic, liu2023reflect, liu2024self, huang2022inner}. Previous approaches, such as probability inference~\cite{diehl2022did}, scene graphs~\cite{das2021semantic}, neural-symbolic planners~\cite{cornelio2024recover}, and purely learning-based policies~\cite{inceoglu2021fino}, have been limited in their ability to address a wide range of failure scenarios and often lack generalizability. Recent efforts have focused on leveraging human feedback to correct robot failures and train policies~\cite{shi2024yell,zha2023distilling,liang2024learning,shinn2024reflexion}, but these approaches are not scalable. Autonomous failure detection and recovery using foundational models~\cite{liu2023reflect, xiong2024aic, guan2024task, ming2023hicrisp, guo2023doremi} offer the potential to detect and explain a broader range of failure scenarios without assumptions about task configuration or failure type, thanks to the strong common-sense reasoning capabilities of foundational models. However, many of these models either rely on extensive fine-tuning~\cite{xiong2024aic}, underutilize the latest Vision-Language Models (VLMs)\cite{liu2023reflect, ming2023hicrisp}, or focus solely on task-level failure explanation while neglecting motion-level execution errors\cite{guan2024task, guo2023doremi}. Our work aims to design methods that facilitate the easy adoption of VLMs for both task-level and motion-level failure detection and recovery.

\subsection{Task and Motion Planning with Foundational Models} 
In recent years, LLMs has emerged as powerful tools for understanding and analyzing high-level task instructions, enabling executable task planning for robots~\cite{ahn2022can, huang2022language, huang2022inner, yao2022react, li2023camel, 10161317}. One inherent limitation of LLMs is their reliance on language input, necessitating the translation of multisensory observations (RGB-D, audio, robot states) into language summaries~\cite{liu2023reflect}. Additionally, 3D spatial reasoning is another barrier preventing the use of LLMs for low-level motion planning and control in robotics~\cite{shi2024yell}. To address these challenges, MLLMs have been developed to handle text, vision, SE(3) pose and other sensory information, allowing for more complex robot control~\cite{yuan2024robopoint, driess2023palm, brohan2023rt, chen2024spatialvlm, liu2024visual, xiong2024aic}. However, these models come with significantly higher training costs due to the need for grounding various data sources. Furthermore, researchers are exploring the use of foundational models to generate value maps for motion planning~\cite{huang2023voxposer}, create reward functions for reinforcement learning techniques~\cite{ma2023eureka}, and write control code for robotics~\cite{vemprala2024chatgpt}, aiming to achieve effective low-level planning and manipulation without expensive retraining. \textcolor{red}{We can add more works about prompt refine.}

%RetroFormer~\cite{yao2023retroformer}introduces a framework to bolster LLMs-based agents by refining prompts based on environment feedback. We refine prompts based on error detection and recovery correctness and efficiency.
